Stabilised Asynchronous Fast Adaptive Composite Multigrid using Additive Damping

Multigrid solvers face multiple challenges on parallel computers. Two fundamental ones read as follows: Multiplicative solvers issue coarse grid solves which exhibit low concurrency and many multigrid implementations suffer from an expensive coarse grid identification phase plus adaptive mesh refinement overhead. We propose a new additive multigrid variant for spacetrees, i.e. meshes as they are constructed from octrees and quadtrees: It is an additive scheme, i.e. all multigrid resolution levels are updated concurrently. This ensures a high concurrency level, while the transfer operators between the mesh levels can still be constructed algebraically. The novel flavour of the additive scheme is an augmentation of the solver with an additive, auxiliary damping parameter per grid level per vertex that is in turn constructed through the next coarser level---an idea which utilises smoothed aggregation principles or the motivation behind AFACx: Per level, we solve an additional equation whose purpose is to damp too aggressive solution updates per vertex which would otherwise, in combination with all the other levels, yield an overcorrection and, eventually, oscillations. This additional equation is constructed additively as well, i.e. is once more solved concurrently to all other equations. This yields improved stability, closer to what is seen with multiplicative schemes, while pipelining techniques help us to write down the additive solver with single-touch semantics for dynamically adaptive meshes.

==> 08e_circular_subdomains.tex <==

\begin{figure}
 \begin{center}
   \includegraphics[width=0.21\textwidth]{illustrations/CircleTrimmed.pdf}
   \includegraphics[width=0.39\textwidth]{results/08-AMR-Graphs/Circle1OrderL2.pdf}
   \includegraphics[width=0.39\textwidth]{results/08-AMR-Graphs/Circle3OrderL2.pdf}
   \\
   \includegraphics[width=0.39\textwidth]{results/08-AMR-Graphs/Circle1OrderLInf.pdf}
   \includegraphics[width=0.39\textwidth]{results/08-AMR-Graphs/Circle3OrderLInf.pdf}
 \end{center}
 \caption{
   Typical adaptive mesh for a setup where the regions with different
   material parameter $\epsilon $ are not axis-aligned.
   One order of magnitude differences in the material parameter (centre)
   vs.~three orders of magnitude (right).
   \label{figure:Poisson:adaptive-grid:circle-solvers}
 }
\end{figure}


We close our experimental setups with a circular subdomain setup (Figure
\ref{figure:Poisson:adaptive-grid:circle-solvers}).
Similar to the deformed checkerboard setup (Figure
\ref{figure:Poisson:adaptive-grid:angled-lines-solvers})
the discontinuity is neither axis aligned or axis orientated.
Refinement occurs in an approximation of a circle
around this discontinuity but will never be able to accurately match it.
The non-linear boundary further challenges all tested solvers.

Small variations of $\epsilon$ can be handled by
all three solvers. 
A decrease in convergence is seen
when not equipped with BoxMG however (Figure
\ref{figure:Poisson:adaptive-grid:circle-solvers}).

This convergence does not last however.
Merely increasing the jump by an order of magnitude
causes additive multigrid and BPX to diverge
without the presence of BoxMG.
Other setups fare better and do not diverge.
However the observed rate of convergence
becomes slow, effectively to the point of non-convergence.
For a jump of three orders of magnitude after
90 iterations all non-diverging setups
report a normalised residual decrease of between
five and six orders of magnitude.

The benefit of adaFACx can be seen to be 
similar to the benefit of BoxMG
but neither are well suited to this setup.

==> algorithm-adAFAC-Jac-alternative-notation.tex <==
\begin{algorithm}%\vspace{-2.5mm}
  \caption{Blueprint of one sweep of the our adAFAC-Jac without AMR. 
  $R^{i}$ or $P^{i}$ denote the recursive application of the restriction or
  prolongation, respectively.
  $\widetilde{R}^{i}$ applies $R$ $(i-1)$ times,
  followed by an application of one smoothed operator.
  $b_f$ is the right hand side of the fine grid equation.
  \label{algorithm:adAFAC:Jac}
  }
    \begin{algorithmic}
    \Function{adAFAC-Jac}{}
    	\State $r _{\ell _{max}} \gets b_f - A_{\ell _{max}} u_{\ell
    	_{max}} $
    	\ForAll {$\ell_{min} \leq \ell \leq \ell _{max}$}
    		\State ${b_\ell } \gets R^{\ell _{max} - \ell} r _{\ell _{max}}$
    		\Comment{Restrict fine grid residual to grid level $\ell $} 
    	\EndFor	
    	%The helper grid space is undefined on the finest grid
    	%\ForAll {$\ell_{min} < \ell < \ell _{max}$}
    	\ForAll {$\ell_{min} \leq \ell < \ell _{max}$}
    		\State ${\widetilde{b}_{\ell }} \gets \widetilde{R}^{\ell _{max} - \ell} r _{\ell _{max}}$ 
    		\Comment{Additional restriction residual into additional grid space}
    	\EndFor	
    	%\ForAll {Additional helper grid space, k}
    	%\For {l $\neq$ f}
    	\ForAll {$\ell_{min} < \ell \leq \ell _{max}$}
    		\State ${{c_\ell } \gets 0};$ ${{\widetilde{c}_\ell } \gets 0}$
    		\Comment Initial ``guess'' for correction and damping parameter
    		\State \Call{jacobi}{$A_\ell c_\ell = b_\ell, \omega $} 
    		\Comment Iterate of correction equation stored in $c_\ell $
    		\State \Call{jacobi}{$A_{\ell -1}
    		\widetilde{c}_{\ell -1} = \widetilde{b}_{\ell -1} , \widetilde{\omega} $} 
    		\Comment Iterate of corresponding damping
    		equation (one level coarser)
    	\EndFor
   		\State ${{c_{\ell _{min}} } \gets 0}$
   		\State \Call{jacobi}{$A_{\ell _{min}} c_{\ell _{min}} = b_{\ell _{min}},
   		\omega $}
   		\comment Coarsest grid update (no additional damping performed)
  		%\State \Call{Smooth}{$A_fu_f=b_f$} 
    	%\ForAll  {Grid space, k}
    	%	\State ${u_c}={u_c} + {{I^c_k}{u_k} - {\widetilde{I}^c_k}{\widetilde{u}_k}}$
    	%\EndFor
    		%\State ${u_c}={u_c}+{I^c_0}{u_0}+\sum_{k=1}^{l_{max}} {{I^c_k}{u_k} - {\widetilde{I}^c_k}{\widetilde{u}_k}}$
  		%\State ${u_f} \gets {u_f}+{P^f_0}{c_0}+\sum_{l=1}^{f} {{P^f_l}{c_l} -
  		%{P^f_l}{\widetilde{c}_l}}$
  		\State $ u_{\ell _{max}} \gets u_{\ell _{max}} + c_{\ell
  		_{min}} + \sum^{{\ell _{max}}}_{\ell = {\ell _{min -1}}} {P^{\ell _{max} - \ell}{c_\ell }
  		- P^{\ell _{max} - (\ell-1)}{\widetilde{c}_{\ell-1}}}$ 
    \EndFunction
    \end{algorithmic}
\end{algorithm}%\vspace{-2.5mm}


==> algorithm-adAFAC-PI-alternative-notation.tex <==
\begin{algorithm}%\vspace{-2.5mm}
  \caption{Blueprint of our adAFAC-PI without AMR. 
  $R^{i}$ or $P^{i}$ denote the recursive application of the single level restriction or
  prolongation, $R$ or $P$, respectively.
  $I$ is the injection operator.
  $b_f$ is the right hand side of the fine grid equation.
  \label{algorithm:adAFAC:PI}
  }
    \begin{algorithmic}
    \Function{adAFAC-PI}{}
    	\State $r _{\ell _{max}} \gets b_f - A_{\ell _{max}} u_{\ell
    	_{max}} $
    	\ForAll {$\ell_{min} \leq \ell \leq \ell _{max}$}
    		\State ${b_\ell } \gets R^{\ell _{max} - \ell} r _{\ell _{max}}$
    		\Comment{Restrict fine grid residual to grid level $\ell $} 
    	\EndFor
    	\ForAll {$\ell_{min} < \ell \leq \ell _{max}$}
    		\State ${{c_\ell } \gets 0};$ ${{\widetilde{c}_\ell } \gets 0}$
    		\Comment Initial ``guesses'' for corrections
    		\State \Call{jacobi}{$A_\ell c_\ell = b_\ell, \omega $} 
    		\Comment Iterate of correction equation stored in $c_\ell $
    		\State ${\widetilde{c}_\ell } \gets  PI{c_\ell }  $
    		\Comment Computation of localised damping for $c_\ell $
    	\EndFor
   		\State ${{c_{\ell _{min}} } \gets 0}$
   		\State \Call{jacobi}{$A_{\ell _{min}} c_{\ell _{min}} = b_{\ell _{min}},
   		\omega $}
   		\comment Coarsest grid update (no additional damping performed)
  		%\State \Call{Smooth}{$A_fu_f=b_f$} 
    	%\ForAll  {Grid space, k}
    	%	\State ${u_c}={u_c} + {{I^c_k}{u_k} - {\widetilde{I}^c_k}{\widetilde{u}_k}}$
    	%\EndFor
    		%\State ${u_c}={u_c}+{I^c_0}{u_0}+\sum_{k=1}^{l_{max}} {{I^c_k}{u_k} - {\widetilde{I}^c_k}{\widetilde{u}_k}}$
  		%\State ${u_f} \gets {u_f}+{P^f_0}{c_0}+\sum_{l=1}^{f} {{P^f_l}{c_l} -
  		%{P^f_l}{\widetilde{c}_l}}$
  		\State $ u_{\ell _{max}} \gets u_{\ell _{max}} + c_{\ell
  		_{min}} + \sum^{{\ell _{max }}}_{\ell = {\ell _{min-1}}} {P^{\ell _{max} - \ell}{c_\ell }
  		- P^{\ell _{max} - \ell}{\widetilde{c}_\ell}}$ 
    \EndFunction
    \end{algorithmic}
\end{algorithm}%\vspace{-2.5mm}

